Fair Anomaly Detection For Imbalanced Groups

Anomaly detection (AD) has been widely studied for decades in many real-world applications, including fraud detection in finance, and intrusion detection for cybersecurity, etc. Due to the imbalanced nature between protected and unprotected groups and the imbalanced distributions of normal examples and anomalies, the learning objectives of most existing anomaly detection methods tend to solely concentrate on the dominating unprotected group. Thus, it has been recognized by many researchers about the significance of ensuring model fairness in anomaly detection. However, the existing fair anomaly detection methods tend to erroneously label most normal examples from the protected group as anomalies in the imbalanced scenario where the unprotected group is more abundant than the protected group. This phenomenon is caused by the improper design of learning objectives, which statistically focus on learning the frequent patterns (i.e., the unprotected group) while overlooking the under-represented patterns (i.e., the protected group). To address these issues, we propose FairAD, a fairness-aware anomaly detection method targeting the imbalanced scenario. It consists of a fairness-aware contrastive learning module and a rebalancing autoencoder module to ensure fairness and handle the imbalanced data issue, respectively. Moreover, we provide the theoretical analysis that shows our proposed contrastive learning regularization guarantees group fairness. Empirical studies demonstrate the effectiveness and efficiency of FairAD across multiple real-world datasets.

==> 2_related.tex <==
\section{Related Work}
\label{sec:related}
In this section, we briefly review the related work on unsupervised anomaly detection and fair machine learning. Due to limited space, the detailed related work could be found in Appendix~\ref{related_work}.\\
\textbf{Unsupervised Anomaly Detection.} 
Anomaly detection has been widely studied for decades in many real-world applications, including fraud detection in the finance domain~\cite{DBLP:journals/compsec/WestB16, DBLP:journals/access/HuangMYC18}, pathology analysis in the medical domain~\cite{DBLP:journals/bmcbi/FaustXHGVDD18, DBLP:journals/access/ShvetsovaBFSD21}, intrusion detection for cyber-security~\cite{DBLP:journals/jnca/LiaoLLT13, DBLP:journals/ett/AhmadKSAA21}, and fault detection in safety-critical systems~\cite{DBLP:journals/ijsysc/JuTLM21}, etc. Different from these methods, this paper tackles the problem of fairness-aware anomaly detection by mitigating the representation disparity with contrastive learning-based regularization.

\textbf{Fair Machine Learning.}
Fair Machine Learning aims to amend the biased machine learning models to be fair or invariant regarding specific variables. A surge of research in fair machine learning has been done in the machine learning community\cite{DBLP:conf/kdd/KobrenSM19, zemel2013learning, bolukbasi2016man, hashimoto2018fairness, zhang2018mitigating}. The existing fair anomaly detection methods tend to suffer from the representation disparity issue in the imbalanced data scenario. To address this issue, this paper aims to alleviate the issue of representation disparity in the imbalanced data scenario by introducing the rebalancing autoencoder module and fair contrastive regularization.





% \section{Related Work}
% \label{related_work}
% \textbf{Unsupervised Anomaly Detection.} 
% Anomaly detection has been widely studied for decades in many real-world applications, including fraud detection in the finance domain~\cite{DBLP:journals/compsec/WestB16, DBLP:journals/access/HuangMYC18}, pathology analysis in the medical domain~\cite{DBLP:journals/bmcbi/FaustXHGVDD18, DBLP:journals/access/ShvetsovaBFSD21}, intrusion detection for cyber-security~\cite{DBLP:journals/jnca/LiaoLLT13, DBLP:journals/ett/AhmadKSAA21}, and fault detection in safety-critical systems~\cite{DBLP:journals/ijsysc/JuTLM21}, etc. The authors of ~\cite{DBLP:journals/csur/PangSCH21} divide the existing anomaly detection methods into two major branches. The methods~\cite{DBLP:conf/kdd/AudibertMGMZ20, DBLP:conf/icde/ChenDHZZZZ21, DBLP:conf/iccv/HouZZXPZ21, DBLP:conf/aaai/YanZXHH21, DBLP:conf/sdm/WangLMGGLW023} in the first branch aim to learn the patterns for the normal samples by a feature extractor. For instance, \cite{DBLP:conf/kdd/AudibertMGMZ20} is an encoder-decoder anomaly detection method, which learns how to amplify the reconstruction error of anomalies with adversarial training; \cite{DBLP:conf/icde/ChenDHZZZZ21} proposes a GAN-based autoencoder model to learn the normal pattern of multivariate time series, and detect anomalies by selecting the samples with the higher reconstruction error. The second branch aims at learning scalar anomaly scores in an end-to-end fashion~\cite{DBLP:conf/iclr/SohnLYJP21, DBLP:conf/icml/LiCCWTZ23, DBLP:conf/nips/JiangLWNWLWZ22}. Notably, the authors of \cite{DBLP:conf/iclr/SohnLYJP21} combine distribution-augmented contrastive regularization with a one-class classifier to detect anomalies; 
% % \cite{DBLP:conf/icml/LiCCWTZ23} propose a time series anomaly detection method by extracting a group of prototypes and learning the diverse normal patterns with a generative model. 
% Different from these methods, this paper tackles the problem of fairness-aware anomaly detection by mitigating the representation disparity with contrastive learning-based regularization.

% \textbf{Fair Machine Learning.}
% Fair Machine Learning aims to amend the biased machine learning models to be fair or invariant regarding specific variables. A surge of research in fair machine learning has been done in the machine learning community\cite{DBLP:conf/kdd/KobrenSM19, zemel2013learning, bolukbasi2016man, hashimoto2018fairness, zhang2018mitigating}. For example, \cite{zemel2013learning} presents a learning algorithm for fair classification by enforcing group fairness and individual fairness in the obtained data representation;  \cite{bolukbasi2016man} proposes approaches to quantify and reduce bias in word embedding vectors that are trained from real-world data; in~\cite{hashimoto2018fairness}, the authors develop a robust optimization framework that minimizes the worst case risk over all distributions and preserves the minority group in an imbalanced data set; in~\cite{zhang2018mitigating}, the authors present an adversarial-learning based framework for mitigating the undesired bias in modern machine learning models. In the field of fair anomaly detection, \cite{DBLP:conf/fat/ZhangD21} utilizes the adversarial generative nets to ensure group fairness and use one-class classification to detect the anomalies; \cite{DBLP:conf/kdd/SongLL21} introduces fairness adversarial training and proposes a novel dynamic weight to reduce the negative impacts from outlier points. The existing fair anomaly detection methods~\cite{DBLP:conf/kdd/SongLL21, DBLP:conf/fat/ZhangD21, DBLP:conf/iccv/FioresiDS23} tend to suffer from the representation disparity issue in the imbalanced data scenario. To address this issue, this paper aims to alleviate the issue of representation disparity in the imbalanced data scenario by introducing the rebalancing autoencoder module and maximizing the uniformity of the samples in the latent space via contrastive learning regularization.

==> 8_impact.tex <==
\section{Broader Impact}
This paper proposes a fairness-aware anomaly detection, which aims to provide fair results when the algorithm is applied to detect anomalies. By embedding fairness into anomaly detection algorithms, this work contributes to reducing bias and discrimination in AI applications, ensuring that technologies serve diverse populations equitably. In sectors such as finance, healthcare, and law enforcement, where anomaly detection plays a crucial role in identifying fraud, diseases, and criminal activities, incorporating fairness principles can prevent the perpetuation of historical biases and protect vulnerable groups from unjust outcomes. Furthermore, by advancing fairness in AI, this research aligns with global efforts to promote ethics in technology development, fostering trust between AI systems and their users. 
